Binary Error-Correcting Codes with Minimal Noiseless Feedback

In the setting of error-correcting codes with feedback, Alice wishes to communicate a $k$-bit message $x$ to Bob by sending a sequence of bits over a channel while noiselessly receiving feedback from Bob. It has been long known (Berlekamp, 1964) that in this model, Bob can still correctly determine $x$ even if $\approx \frac13$ of Alice's bits are flipped adversarially. This improves upon the classical setting without feedback, where recovery is not possible for error fractions exceeding $\frac14$. The original feedback setting assumes that after transmitting each bit, Alice knows (via feedback) what bit Bob received. In this work, our focus in on the limited feedback model, where Bob is only allowed to send a few bits at a small number of pre-designated points in the protocol. For any desired $\epsilon > 0$, we construct a coding scheme that tolerates a fraction $ 1/3-\epsilon$ of bit flips relying only on $O_\epsilon(\log k)$ bits of feedback from Bob sent in a fixed $O_\epsilon(1)$ number of rounds. We complement this with a matching lower bound showing that $\Omega(\log k)$ bits of feedback are necessary to recover from an error fraction exceeding $1/4$ (the threshold without any feedback), and for schemes resilient to a fraction $1/3-\epsilon$ of bit flips, the number of rounds must grow as $\epsilon \to 0$. We also study (and resolve) the question for the simpler model of erasures. We show that $O_\epsilon(\log k)$ bits of feedback spread over $O_\epsilon(1)$ rounds suffice to tolerate a fraction $(1-\epsilon)$ of erasures. Likewise, our $\Omega(\log k)$ lower bound applies for erasure fractions exceeding $1/2$, and an increasing number of rounds are required as the erasure fraction approaches $1$.

==> acknowledgements.tex <==
\section{Acknowledgments}

Meghal Gupta is supported by a Chancellor's fellowship from UC Berkeley. \mnote{add your fellowships. also anyone we want to thank? Rachel did you discuss the problem with Yael?}

==> erasure-protocol/ecc.tex <==
\subsection{The error-correcting Code}

In this section, we will use an error-correcting code with a list-decoding property in the face of erasures.

\begin{theorem}\cite{Guruswami03} \label{thm:erasure-list-ECC}
    There is an explicit family of maps $\ECC = \{ \ECC_k : \{ 0, 1 \}^k \rightarrow \{ 0, 1 \}^{n_0(k)} \}_{k \in \bbN}$ with the following properties:
    \begin{itemize}
    \item $n_0 = O_\epsilon(k)$.
    \item 
        For all $k$ and $x \in \{ 0, 1 \}^k$, if $< 1 - \epsilon$ of $\ECC(x)$ is erased, there is a polynomial time algorithm that outputs $L_\epsilon = O(1/\epsilon) \ge 1/\epsilon$ values $x_1, \dots, x_{L_\epsilon} \in \{ 0, 1 \}^k$ with the guarantee that $x \in \{ x_1, \dots, x_{L_\epsilon} \}$. 
    \end{itemize}
\end{theorem}
\mnote{as we defined things in the other sections/previous papers, we called the family $\ECC_\epsilon$. lmk which is better. Also $n_0$ vs $M$.}

==> error-protocol/protocol-overview.tex <==
\subsection{Informal Description of the Protocol}

\vnote{It might be best to integrate this section with the earlier overview as there is a fair bit of repetition, incorporating any added important issues addressed here, such as the top two increasing by $2/3$.}

As opposed to Section~\ref{sec:overview-error}, this description focuses more on the exact protocol and technical details. Nonetheless, it is self-contained, and the reader can read this without reading the overview.

Suppose that Alice has input $x \in \{ 0, 1 \}^k$, which she is trying to convey to Bob over constant rounds with $\log{k}$ feedback from Bob.

The main structure of our protocol $\pi$ follows the \emph{coin game} structure used in the work of Spencer and Winkler \cite{SpencerW92}. In this structure, Bob keeps track of coins (counters) and their positions, as described below.

\begin{itemize}
    \item {\bf Coins:} There are $2^k$ coins on a board, each labeled with one of the possible values of Alice's input $\in \{ 0, 1 \}^k$.
    \item {\bf Position:} A coin's position denotes (a lower bound on) the amount of corruption the adversary must've caused to Alice's communication so far if Alice's input were indeed that coin, as a fraction of complete messages (so fully corrupting a message of length $M=M(k)$ means that the coin should be at position $M$).
\end{itemize}

With the view that a coin's position is the total amount of corruption so far if Alice's input had actually been that coin, our goal is to show that at the end of the protocol, at most one coin can have position $< \frac13|\pi|$\footnote{Technically, this should be $\left(\frac13-\epsilon\right)|\pi|$. Throughout the explanation, we omit the $\epsilon$'s.}.

The protocol is divided into a constant number $C$ of \emph{chunks} which are further subdivided into a constant number $R$ of rounds of length $M$. Between rounds (and between chunks), Bob provides Alice with some fixed amount $\Theta(\log{k})$ bits of feedback. 

Throughout the protocol, Alice will follow one of three high level strategies in each chunk for how to encode her message, which Bob decides on at the start of the chunk and tells her as feedback. The first is a fairly simple strategy involving sending the ECC from Definition~\ref{def:ecc}, the second is more complicated and involves the ECC's from Definition~\ref{def:ecc3}, and the third involves Alice just sending a single bit for the whole chunk. We note that Alice and Bob switch between the first two strategies at first, but once they use the third strategy ever, they will continue to do so for the remainder. At the end of every chunk, Bob updates the state of his coin game based on how much corruption there would have been in that chunk had Alice's true input been each coin $y$. Our goal will be to show that at most one coin ends in position $\leq \frac13|\pi|$. 

Now we describe the two strategies Alice and Bob may engage in during a chunk.

\paragraph{Bob tells Alice to use the traditional distance $\frac12$ ECC as in Definition~\ref{def:ecc}.} In this case, Alice sends $\ECC(x)$ to Bob, which is a message of length $RM$. \vnote{What are $R$ and $M$?} Bob sends feedback messages in between, but Alice ignores this, just sending the next $M$ bits of her encoding in every round. (The round structure is not necessary for this strategy, but is included in the overall protocol structure because it is necessary later.) At the end of the chunk Bob wants to update the coin states, moving each coin $y$ by $\Delta(y,\ECC(m))$ where $m$ is the corrupted length $RM$ message of he received throughout the chunk. \vnote{Should be $\Delta(m,\ECC(y))$} Naively, this would take exponential-in-$k$ time, but by list decoding $m$ instead, Bob can update only the $L_\epsilon$ coins $y$ with small $\Delta(y,\ECC(m))$ explicitly, and update the rest by $\approx \frac12 RM$ instead (which is approximately a lower bound on the true distance due to the list-decoding guarantee of Definition~\ref{def:ecc}. Then, he only needs to track a constant number of the updates made that chunk explicitly. Since there are only a constant number of chunks, overall he is only tracking a constant number of updates explicitly. The exact data structure used for the coin game is described in Definition~\ref{def:coin-game}. 

The fact that all but a constant number of the coins increase by $\frac12RM$ in position is useful for another reason. Because we only need to guarantee some coin exceeds $\frac13|\pi|$ at the end of the protocol, increasing the average element by $\frac12RM$ in every chunk is well on our way to this goal.

However, there may be a small number of coins that do not increase by at least $\frac12RM$ in value. For example, the adversary may choose a corruption pattern so two (or even three) of the coins' positions increase by only $\frac14RM$ in every chunk. Indeed, if Bob tells Alice only to send $\ECC(x)$ for the entirety of the protocol, this is an attack that succeeds with only $\frac14$-fraction corruption of the protocol.

Our hope is to use the second ECC to separate out these few coins that are increasing too slowly. Remember also that most coins were increasing each chunk by $\frac12RM$, which is actually higher than the required increase of $\frac13RM$ per chunk---the slack from here is what makes the second ECC able to compensate for the shortcomings of this first ECC. More formally, let $\posx(i)$ be the position of the coin with the $i$'th smallest position value. Bob switches Alice to using the second ECC whenever $\posx(3)\ll\posx(L)$ for some large constant $L$ ($L$ depends on the round number, but we ignore that for now, and $\ll$ means ``less than by at least $10\epsilon |\pi|$'').

\paragraph{Bob tells Alice to play the coin minigame using the special ECC as in Definition~\ref{def:ecc3}.} Recall that our main goal here is to separate out Bob's first $L$ coins further while using the fact that coins $L$ through $2^k$ have increased by more than necessary so far. However, there's a difficulty in this: Bob singling out a set of $L$ (the first $L$ coins) elements requires $O(k)$ bits of communication and we only have $O(\log{k})$ bits. Therefore, Bob can't even tell Alice what these $L$ elements are. However, he can instead tell her a partition $P$ into $L$ sets of her $2^k$ possible inputs into sets so that coins $1\ldots L$ are in different sets (essentially, he does this with only $O_\epsilon(\log{k})$ bits by giving her a constant-sized list of indices on which coins $1\ldots L$ all differ). He specifies this at the start of the chunk using $\partition$ so the description is only $O_\epsilon(\log{k})$ bits. \vnote{$\partition$ notation might be too specific for the overview...}

Now we describe what the parties actually do during the chunk -- they play a new instantiation of a coin game, called the \emph{coin minigame}. Bob's new instantiation of a coin minigame has its coins as the $L$ sets of $P$, all starting at position $0$. He sends this partition over to Alice as explained above. Before each round, he orders the sets in $P$ according to their positions in the coin minigame as $S(1)\ldots S(L)$, and sends Alice $f$ specifying the partition $\{S(1)\}, \{S(2),S(4),S(6)\ldots\}, \{S(3),S(5),S(7)\ldots\}$ labeled $\{1,2,3\}$ respectively. Then, Alice sends him $\ECC[P,f](x)$. \vnote{Where is this ECC defined?} This ECC has the properties that elements in different (coarsened) partitions are distance $\frac{2}{3} M$ apart and elements in $S(1)$ are still distance $\frac13$ apart. Then, Bob updates the coin minigame by moving a set $S$ by the minimum amount that any element of the set had moved in that round ($\min_{y\in S}\Delta(m,\C(y))$). 

At the end of the chunk, Bob discards the coin minigame and updates the main coin game according to a lower bound on how much corruption each coin required given the messages Bob received. Specifically, he moves the first $L$ coins by how much the corresponding set in $P$ moved, and moves all but a constant number of the remaining coins by $\frac13RM$. We show in Section~\ref{sec:minigame-analysis} that this is actually a lower bound on the corruption\footnote{This is actually one of subtler points, since it heavily constrains the design of $\ECC[s,f]$. It is, for example why the odd-even coin game method of Spencer and Winkler \cite{SpencerW92} does not adapt to our situation, as well as many other adaptive question-asking schemes one may play with.}! (The constant number of coins that don't have a lower bound of $\frac13RM$ on the corruption just move by how much their corresponding set in $P$ moved.)

With these movements, it turns out the new sum of $\posx(1)+\posx(2)$ is at least $\frac23RM$ higher than at the start of the chunk and the new sum of $\posx(1)+\posx(2)+\posx(3)$ is at least $RM$ higher. This crucially requires that the first three coins now must have all been in the first $L$ coins at the start of the chunk -- which holds because $\posx(L)\gg\posx(3)$ at the start of the chunk. Then, analysis of the minigame shows any pair of coins increases by at least $\frac23RM$ and any triple by at least $RM$. Moreover, since all but a constant number of the remaining coins were updated by $\frac13RM$, we also have that $x_L$ increased by $\frac13RM$ (technically, this new $L$ is slightly larger than the $L$ from the start of the chunk, and in the formal protocol we scale $L$ with the round number).

We write down a key potential function: $\posx(1)+\posx(2)+\posx(L)$. As we just showed, this quantity increases by at least $RM$ per round on average when playing the coin minigame. Notice that this actually also holds when Alice sends a normal ECC -- all but a small constant number of the coins increase by $\frac12M$ and so $\posx(1)+\posx(2)$ increases by $\frac12M$ and $\posx(L)$ increases by $\frac12M$. Because Alice transitions to playing the coin minigame whenever $\posx(3)\ll\posx(L)$, coin $3$ and coin $L$ remain close throughout the protocol (unless the adversary is making particularly suboptimal corruptions), and so on average, the potential $\posx(1)+\posx(2)+\posx(3)$ increases by $RM$. \mnote{I think i explained this paragraph a little badly.}

\paragraph{Bob tells Alice to send a single bit.} We are almost done at this point -- however with only the potential $\posx(1)+\posx(2)+\posx(3)$ increasing by $RM$ per chunk, it's possible for $\posx(3)$ to be large while $\posx(2)$ fails to exceed $\frac13|\pi|$ by the end of the protocol. Thus, when $\posx(3)$ exceeds $\frac13|\pi|$ (and so only coins $1$ and $2$ are possibilities for Alice's input), Bob sends Alice a single index on which coin $1$ and coin $2$ differ. Then, $\posx(1)+\posx(2)$ itself will increase by $RM$ per chunk until $\posx(2)$ exceeds $\frac13|\pi|$ as well. The final calculation in Section~\ref{sec:analysis-error} shows that coin $\posx(2)>\frac13|\pi|$ by the end of the protocol.

==> old/1.3-protocol/analysis.tex <==
\subsection{Analysis}

In this section, we analyze Protocol~\ref{prot:1/3-k}. Our main theorem is the following:

\begin{theorem} \label{thm:1/3-k}
    Protocol~\ref{prot:1/3-k} has $O_\epsilon(1)$ rounds and is resilient against $\left( \frac13 - \frac43 \epsilon \right)$ errors.
\end{theorem}

\subsubsection{A Property About Triples}

We consider triples of distinct coins by referencing their relative positions on the board. That is, we will represent triples by pairwise distinct $i, j, k \in [2^k]$. We will consider triples up to permutation, so for instance the triple $(i, j, k)$ denotes the same triple as $(k, i, j)$. When it is convenient to do so, we will typically represent a triple by $(i, j, k)$ where $i < j < k$. We may also drop the parenthesis, so we may denote triples by $ijk$.

We define the partial ordering $(i, j, k) \le (i', j', k')$, where $i < j < k$ and $i' < j' < k'$, if $i \le i'$, $j \le j'$, and $k \le k'$, with strict inequality if $(i, j, k) \not= (i', j', k')$.

We will be interested in the sum of positions of the $i$'th, $j$'th, and $k$'th coins on the board. For $i,j,k \in [2^k]$, define 
\[ 
    \phi_{ijk}(t) := \pos(x_i^{(t)}; t) + \pos(x_j^{(t)}; t) + \pos(x_k^{(t)}; t),
\]
and let
\[
    \phi(t) := \phi_{123}(t) = \min_{ijk} \phi_{ijk}(t).
\]
In this section, our goal is to show that $\phi(T) \approx T$. 

\paragraph{Bob's update pattern.}

We begin with some observations about Bob's update pattern.

\begin{lemma} \label{lemma:e-properties}
    For any update pattern $(e_1, \dots, e_{2^k})$, the following hold:
    \begin{enumerate}
    \item All except for $L_\epsilon$ values of $e_i$ must be at least $\frac12 - 2\epsilon$. 
    \item $e_{2j-1} + e_{2j} = 1$ for all $i \in [L_\epsilon]$.
    \item If $e_i \ge \frac12 - 2\epsilon$, then for any distinct $j, k \neq i$ it holds that $e_i + e_j + e_k \ge 1 - 3\epsilon$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    The first property follows from list decoding, and the second property follows from the distance properties of our ECC (see Theorem~\ref{thm:ECC-list-decoding} \rnote{fill in theorem once written}).
    
    For the third property, note that all pairs of codewords are distance $\ge \frac12 - \epsilon$ apart. Thus, in particular, $e_j + e_k \ge \frac12 - \epsilon$. Then, $e_i \ge \frac12 - 2\epsilon \implies e_i + e_j + e_k \ge 1 - 3\epsilon$. In particular, there are at most $O_\epsilon(1)$ triples $(i,j,k)$ for which $e_i + e_j + e_k < 1 - 3\epsilon$.
\end{proof}

\begin{lemma} \label{lemma:triple-bijection}
    For each triple $(i, j, k)$ such that $e_i + e_j + e_k < 1-3\epsilon$, there is another triple $f(ijk) = (i', j', k') < (i, j, k)$ satisfying:
    \begin{enumerate}
        \item $(e_i + e_j + e_k) + (e_{i'} + e_{j'} + e_{k'}) \ge 2 - 6\epsilon$.
        \item No two triples $(i, j, k) \not= (\hat{i}, \hat{j}, \hat{k})$ satisfying $e_i + e_j + e_k < 1-3\epsilon$ and $e_{\hat{i}} + e_{\hat{j}} + e_{\hat{k}} < 1 - 3\epsilon$ have the same associated triple, that is, $f(ijk) \not= f(\hat{i}\hat{j}\hat{k})$. 
    \end{enumerate}
\end{lemma}

\begin{proof}
    Suppose that the update pattern $(e_1, \dots, e_{2^k})$ is obtained from a message $m$ in round $t$.
    
    Consider a triple $i < j < k$ for which $e_i + e_j + e_k < 1 - 3\epsilon$. Note by Lemma~\ref{lemma:e-properties} that it must hold that $e_i, e_j, e_k < \frac12 - 2\epsilon$, or that $x_i^{(t-1)}, x_j^{(t-1)}, x_k^{(t-1)} \in Y_t$. If we write $Y_t = \{ y_{t,i} \}_{i \in [\ell_t]}$ with $\pos(y_{t,1}; t-1) < \pos(y_{t,2}; t-1) < \dots, < \pos(y_{t,\ell_t}; t-1)$, let $a < b < c \in [\ell_t]$ be such that $x_i^{(t-1)} = y_{t,a}$, $x_j^{(t-1)} = y_{t,b}$, and $x_k^{(t-1)} = y_{t,c}$.
    
    We construct the triple $(i', j', k')$ as follows:
    \begin{itemize}
        \item $i' = i$.
        \item $j'$ is either $2(b-1)-1$ or $2(b-1)$, whichever satisfies $e_{j'} \ge \frac12$. Note that either $j' = 2(b-1)-1$ or $j' = 2(b-1)$ must satisfy this property, since $e_{2(b-1)-1} + e_{2(b-1)} = 1$.
        \item $k'$ is either $2(c-1)-1$ or $2(c-1)$, whichever satisfies $e_{k'} \ge \frac12$. 
    \end{itemize}
    
    Then, it holds that 
    \begin{align*}
        (e_i + e_j + e_k) + (e_{i'} + e_{j'} + e_{k'}) &\ge (e_i + e_j) + (e_i + e_k) + \frac12 + \frac12 \\
        &\ge \left( \frac12 - \epsilon \right) + \left( \frac12 - \epsilon \right) + 1 \\
        &\ge 2 - 2\epsilon \\
        &\ge 2 - 6\epsilon.
    \end{align*}
    
    Next, we prove that $(i', j', k') < (i, j, k)$. To see this, notice that $j' < j$ and $k' < k$, since $j' \le 2(b-1)$ and $j > 2(b-1)$, the latter of which holds because $j$ must be the $b$'th smallest index for which $\frac{\Delta(\ECC_t(e_j), m)}{n_0} < \frac12 - 2\epsilon$, and out of each of the first $L_\epsilon$ pairs of indices at most one of each pair can have this property. The same logic holds for $k' < k$. 
    
    Finally, to see uniqueness, notice that to reconstruct $(i, j, k)$ from $(i', j', k')$, define $b = \lceil \frac{j'}{2} \rceil$ and $c = \lceil \frac{k'}{2} \rceil$, and pick $j$ and $k$ to be the $b$'th and $c$'th smallest positions of the list decoding possibilities, and take $i = i'$. 
\end{proof}

\paragraph{Showing $\phi(T) \approx T$.}

Now we will show that $\phi(T) \approx T$. Recall that $\phi(T) = 123(T) = \pos(x_1^{(T)}; T) + \pos(x_2^{(T)}; T) + \pos(x_3^{(T)}; T)$. 

Consider the following new coin game: instead of each coin corresponding to a possible input $\in \{ 0, 1 \}^k$, each coin in Coin Game~\ref{prot:coingame-B} will correspond to \emph{three} different coins. Its position is the sum of the positions of the three coins in Coin Game~\ref{prot:coingame-A}. 

\coingame{Coin Game}{}{coingame-B}{
    \begin{itemize}
    \item 
        {\bf Coins:} There are $\binom{2^k}{3}$ coins, corresponding to all (unordered) triples of inputs $\in \{ 0, 1 \}^k$.
    \item 
        {\bf Position:} The position of a coin corresponding to $(y,z,w)$ is the sum of the positions of the coins in Coin Game~\ref{prot:coingame-A}.
    \item 
        {\bf Notation:} We refer to the coin $(x_i^{(t)}, x_j^{(t)}, x_k^{(t)})$ as $x_{ijk}^{(t)}$ for short. After round $t$, note that the coin $x_{ijk}^{(t)}$ is at position $\phi_{ijk}(t)$. 
    \item {\bf Updates:} In round $t$, Bob will update coin $x_{ijk}^{(t-1)}$ by $e_{ijk} := e_i + e_j + e_k$. 
    \end{itemize}
}

The goal is then to show that at time $T$, the position of the first coin in Coin Game~\ref{prot:coingame-B} is at least $( \frac13 - \frac43 \epsilon) \cdot T$. 

\begin{lemma} \label{lemma:smaller-updates}
    Suppose that Bob reaches a final board configuration in Coin Game~\ref{prot:coingame-B} via a sequence of updates $\left\{ \{ e_{ijk}^{(t)} \}_{i,j,k \in \binom{2^k}{3}} \right\}_{t \in [T]}$. If for some $t$ we replace $\{ e_{ijk}^{(t)} \}_{i,j,k \in \binom{2^k}{3}}$ by $\{ f_{ijk}^{(t)} \}_{i,j,k \in \binom{2^k}{3}}$, where $f_{ijk}^{(t)} \le e_{ijk}^{(t)}$ for all $i,j,k$, then the resulting value of $\phi(T)$, which we denote by $\phi'(T)$, is at most the value of $\phi(T)$ in the original experiment.
\end{lemma}

\begin{proof}
    \rnote{TODO}
\end{proof}

By Lemma~\ref{lemma:smaller-updates}, in the analysis we can replace any updates Bob does with smaller updates since the resulting $\phi(T)$ will be no bigger than the original value.

In particular, let us choose update weights $\{ f_{ijk}^{(t)} \}_{i,j,k \in \binom{2^k}{3}}$ satisfying the following property: for any $ijk$ and $t$ with $e_{ijk}^{(t)} < 1 - 3\epsilon$, let $i'j'k' < ijk$ be the corresponding triple from Lemma~\ref{lemma:triple-bijection}. Then we have $f_{ijk}^{(t)} = e_{ijk}^{(t)}$ and $f_{i'j'k'}^{(t)} = 2 - 6\epsilon - e_{ijk}^{(t)}$. For all other triples $ijk$, we have $f_{ijk}^{(t)} = 1 - 3\epsilon$.

Now, consider the following potential function 
\[
    F(t) = \sum_{ijk \in \binom{2^k}{3}} (1 + \epsilon)^{2|\phi_{ijk}(t) - (1-3\epsilon)t|} - \left( \binom{2^k}{3} - T \cdot 2L_\epsilon \right).
\]

Note that at time $t = 0$, all coins are at position $\phi_{ijk}(0) = 0$, so $F(0) = 2TL_\epsilon$. Furthermore, note that at any point at most $2TL_\epsilon$ coins are \emph{not} at position $(1 - 3\epsilon) \cdot T$, since each round at most $2L_\epsilon$ of the coins are moving by $f_{ijk}^{(t)} \not= 1 - 3\epsilon$. Thus, $F(t)$ essentially tracks a term of $(1 + \epsilon)^{2|\phi_{ijk}(t)-(1-3\epsilon)t|}$ for each triple $(x_i^{(t)}, x_j^{(t)}, x_k^{(t)})$ that can ever not be at position $(1 - 3\epsilon) \cdot T$ and disregards the contribution from the rest.

We analyze the effect of an update sequence $\{ f_{ijk}^{(t)} \}_{i,j,k \in \binom{2^k}{3}}$ on the value of $F(t)$. 

\begin{lemma} \label{lemma:Ft}
    $F(t) \le e^{\epsilon^2/2} F(t-1) + 2\epsilon L_\epsilon$.
\end{lemma}

\begin{proof}

    Note that for all but $2TL_\epsilon$ of the triples, the coin will increment its position by $1-3\epsilon$ every round. Thus their contribution to the sum is $1$, and their effect is discounted by the $-\left( \binom{2^k}{3} - T \cdot 2L_\epsilon \right)$ term. We now look at the effect of the remaining $2TL_\epsilon$ terms.
    
    First, any coin that increments by exactly $1-3\epsilon$ will not change its contribution to $F(t)$.
    
    Now, consider a triple $ijk$ with $f_{ijk}^{(t)} < 1 - 3\epsilon$ and its associated triple $i'j'k' < ijk$. Let $f_{ijk}^{(t)} = 1 - 3\epsilon - \delta$ and $f_{i'j'k'}^{(t)} = 1-3\epsilon+\delta$. We remark that $\delta \le \frac14$ (in fact $\delta \le \frac14 - 3\epsilon$) by 3-way list decoding. \rnote{insert a lemma about this, in the above ecc section}
    
    After the update in round $t$, the contribution of the coins $x_{ijk}^{(t-1)}$ and $x_{i'j'k'}^{(t-1)}$ is
    \[
        (1 + \epsilon)^{2|\phi_{ijk}(t-1) - (1-3\epsilon) \cdot (t-1) - \delta|} + (1 + \epsilon)^{2|\phi_{i'j'k'}(t-1) - (1-3\epsilon) \cdot (t-1) + \delta|}. \numberthis \label{eqn:t-contribution}
    \]
    We claim that this is at most 
    \[
        e^{\epsilon^2/2} \cdot \left( (1 + \epsilon)^{2|\phi_{ijk}(t-1) - (1-3\epsilon) \cdot (t-1)|} + (1 + \epsilon)^{2|\phi_{i'j'k'}(t-1) - (1-3\epsilon) \cdot (t-1)|} \right) + 2\epsilon. \numberthis \label{eqn:t-contribution-upper}
    \]
    To see this, we consider two cases. The first is that $\phi_{ijk}(t-1)$ and $\phi_{i'j'k'}(t-1)$ fall on the same side of (are both either greater or less than) $(1-3\epsilon)\cdot (t-1)$, and the farther is at least $\delta$ away. In this case, let $D$ be the larger of $|\phi_{ijk}(t-1) - (1-3\epsilon) \cdot (t-1)|$ and $|\phi_{i'j'k'}(t-1) - (1-3\epsilon) \cdot (t-1)|$, and let $d$ be the smaller. Then recalling that $i'j'k' < ijk$, we have that Equation~\eqref{eqn:t-contribution} is
    \begin{align*}
        (1+\epsilon)^{2(D-\delta)} + (1+\epsilon)^{2(d+\delta)} 
        &\le  \frac{(1+\epsilon)^{2\delta} + (1+\epsilon)^{-2\delta}}{2} \cdot \left( (1+\epsilon)^{2D} + (1+\epsilon)^{2d} \right) \\
        &\le \frac{(1+\epsilon) + (1+\epsilon)^{-1}}{2} \cdot \left( (1+\epsilon)^{2D} + (1+\epsilon)^{2d} \right) \\
        &\le \left( 1 + \frac{\epsilon^2}{2} \right) \cdot \left( (1+\epsilon)^{2D} + (1+\epsilon)^{2d} \right) \\
        &\le e^{\epsilon^2/2} \cdot \left( (1+\epsilon)^{2D} + (1+\epsilon)^{2d} \right) \\
        &\le e^{\epsilon^2/2} \cdot \left( (1+\epsilon)^{2D} + (1+\epsilon)^{2d} \right) + 2\epsilon,
    \end{align*}
    where the first inequality follows by convexity, the second follows from $\delta \le \frac14 \le \frac12$ and by convexity, and the others follow from standard approximation inequalities.
    
    The second case is that $\phi_{ijk}(t-1)$ and $\phi_{i'j'k'}(t-1)$ fall on different sides of $(1-3\epsilon) \cdot (t-1)$, or both are within $\delta$ of $(1-3\epsilon) \cdot (t-1)$. In this case, notice that if one of the distances is greater than $\delta$, then its contribution necessarily must decrease. On the other hand, if its distance is $< \delta$, then at the end of the update, its distance can be at most $2\delta$, so that its new contribution is at most $(1+\epsilon)^{2\cdot 2\delta} \le (1+\epsilon)$, where we use that $\delta \le \frac14$. Meanwhile, its original contribution has to be at least $1$, so the total extra additive contribution is at most $\epsilon$. This holds for both terms, for a total increase in contribution by at most $2\epsilon$. Thus our claim that Equation~\eqref{eqn:t-contribution} is at most Equation~\eqref{eqn:t-contribution-upper} holds for this case as well.
    
    Now, in total, each of the $T \cdot 2L_\epsilon$ terms we track either don't change its contribution, or else can be paired up with another satisfying~\eqref{eqn:t-contribution} $\le$~\eqref{eqn:t-contribution-upper}. In total this gives us that 
    \[
        F(t) \le e^{\epsilon^2/2} F(t-1) + 2\epsilon L_\epsilon.
    \]
\end{proof}

We are now in position to prove our main lemma for this section.

\begin{lemma} \label{lemma:triples}
    For large enough $T = O_\epsilon(1)$ for which $\epsilon^2 T \ge 2 \ln (2TL_\epsilon + 4L_\epsilon/\epsilon)$, it holds that $\phi(T) \ge (1-4\epsilon)\cdot T$. 
\end{lemma}

\begin{proof}
    We solve the recurrence in Lemma~\ref{lemma:Ft} to get that
    \begin{align*}
        F(T) 
        &\le e^{T\epsilon^2/2} \cdot F(0) + 2\epsilon L_\epsilon \cdot \left( e^{(T-1)\epsilon^2/2} + e^{(T-2)\epsilon^2/2} + \dots + 1 \right) \\
        &= e^{T\epsilon^2/2} \cdot 2TL_\epsilon + 2\epsilon L_\epsilon \cdot \frac{e^{T\epsilon^2/2}-1}{e^{\epsilon^2/2}-1} \\
        &\le e^{T\epsilon^2/2} \cdot \left( 2TL_\epsilon + \frac{2\epsilon L_\epsilon}{\epsilon^2/2} \right) \\
        &= e^{T\epsilon^2/2} \cdot \left( 2TL_\epsilon + \frac{4 L_\epsilon}{\epsilon} \right).
    \end{align*}
    Then, we have that
    \begin{align*}
        (1+\epsilon)^{2|\phi(T) - (1-3\epsilon) \cdot T|} &\le F(T) \le e^{T\epsilon^2/2} \cdot \left( 2TL_\epsilon + \frac{4 L_\epsilon}{\epsilon} \right) \\
        \implies 
        2|\phi(T) - (1-3\epsilon) \cdot T| \cdot \ln (1+\epsilon) &\le T\epsilon^2/2 + \ln \left( 2TL_\epsilon + \frac{4 L_\epsilon}{\epsilon} \right) \\
        \implies \phi(T) &\ge (1-3\epsilon) \cdot T - \frac{T\epsilon^2/2 + \ln \left( 2TL_\epsilon + 4L_\epsilon/\epsilon \right)}{2\ln (1+\epsilon)}.
    \end{align*}
    We have that $\ln(1+\epsilon) \ge \frac\epsilon2$, which gives us the inequality
    \begin{align*}
        \phi(T) 
        &\ge (1-3\epsilon) \cdot T - \frac{\epsilon T}{2} + \frac1\epsilon \cdot \ln(2TL_\epsilon + 4L_\epsilon/\epsilon) \\
        &\ge (1 - 4\epsilon) \cdot T,
    \end{align*}
    where the last inequality follows from the assumption in the statement of the lemma.
\end{proof}


\subsubsection{Proof of Theorem~\ref{thm:1/3-k}}

We are now ready to prove Theorem~\ref{thm:1/3-k}. 

\begin{proof}[Proof of Theorem~\ref{thm:1/3-k}]
    Suppose for the sake of contradiction that there is some sequence of messages that Bob could receive such that $\pos(x_1^{(T)}; T), \pos(x_2^{(T)}; T) < \frac{1-4\epsilon}{3} \cdot T$. 
    
    Consider the potential function 
    \[
        \Psi(t) = \pos(x_1^{(t)}; t) + \pos(x_2^{(t)}; t) + \min \left( \pos(x_3^{(t)}; t), \frac{1-4\epsilon}{3} \cdot T \right).
    \]
    According to Lemma~\ref{lemma:triples}, as long as there are still three coins with positions $< \frac{1-4\epsilon}{3} \cdot T$, $\Psi(t)$ increases by $\ge 1 - 4\epsilon$ each round. After the third coin has reached position $\ge \frac{1-4\epsilon}{3} \cdot T$, by assumption we always have that the first two coins both have positions $< \frac{1-4\epsilon}{3} \cdot T$ so there can be no crossover with other coins, thus $\Psi(t)$ increases by $1$ each round since the first two coins' distances must always add up to $1$. Therefore, $\Psi(T) \ge (1-4\epsilon) \cdot T$. But combining with the fact that $\min \left( \pos(x_3^{(t)}; t), \frac{1-4\epsilon}{3} \cdot T \right) \le \frac{1-4\epsilon}{3} \cdot T$, we obtain that
    \[
        \pos(x_1^{(T)}; T) + \pos(x_2^{(T)}; T) \ge \frac{2 - 8\epsilon}{3} \cdot T,
    \]
    which implies that 
    \[
        \pos(x_2^{(T)}; T) \ge \frac{1-4\epsilon}{3} \cdot T,
    \]
    contradiction.
\end{proof}



==> old/1.3-protocol/ecc.tex <==
\subsection{The Error Correcting Code}

In this first section, we will describe the code that Alice will use to encode her input.

\rnote{todo; list-decoding of radius $\frac12 - 2\epsilon$ to list of size $L_\epsilon$; ECC should be $\{ 0, 1 \}^k \rightarrow \{ 0, 1 \}^{n_0}$; total protocol has size $n$}

\begin{definition}[$\ECC$]
    For a given $\epsilon > 0$, we define the error correcting code family $$\ECC_\epsilon= \{ \ECC_{\epsilon,k} : [2^k] \rightarrow \{ 0, 1 \}^{n_0(k)} \}_{k \in \bbN}$$ with the following properties:
    
    \begin{itemize}
    \item $n_0(k)=O_\epsilon(k)$.
    \item For any $i,j \in [2^k]$, 
    \[
        \Delta \big( \ECC_{\epsilon,k}(i), \ECC_{\epsilon,k}(j) \big) \ge \left( \frac12 - \epsilon \right) \cdot n_0(k), \numberthis \label{eqn:ecc-1/2}
    \]
    \item For any odd-numbered $i\in [2^k]$,
    \[
        \Delta \big( \ECC_{\epsilon,k}(i), \ECC_{\epsilon,k}(i+1) \big) = n_0. \numberthis \label{eqn:ecc-1}
    \]
    \rnote{lmao we need to decide if $\Delta$ is absolute distance or relative distance. maybe we should just keep as absolute distance for consistency with the literature} \mnote{yeah i agree with absolute distance}
\end{itemize}
\end{definition}


==> old/1.3-protocol/k-bit-protocol.tex <==
\subsection{ECC with Feedback with Constant Rounds and $O_\epsilon(k)$ Bits of Feedback}


Suppose that Alice has input $x \in \{ 0, 1 \}^k$, which she is trying to convey to Bob over constant rounds with feedback from Bob.

Our protocol will consist of $T = O_\epsilon(1)$ rounds. Bob keeps track of the state of the following coin game. There are $2^k$ coins on a board, corresponding to the possible values of Alice's input $\in \{ 0, 1 \}^k$. A coin's position on the horizontal axis denotes (a lower bound on) the amount of corruption the adversary must've caused to Alice's communication so far if Alice's input were actually that coin, as a fraction of complete messages (so fully corrupting a message means that the coin should be at position $1$). At the beginning of the game, all coins are at position $0$. We denote by $\pos(y; t)$ the position of the coin labeled $y$ after the $t$'th round (that is, Alice has sent her $t$'th message and Bob has updated correspondingly, as we describe in a bit). Also, after any round $t$, let $x_i^{(t)}$ denote the label of the coin that has the $i$'th smallest label, where we break ties arbitrarily. This coin game is summarized in Figure~\ref{prot:coingame-A}.

\coingame{Coin Game}{}{coingame-A}{
    \begin{itemize}
        \item {\bf Coins:} There are $2^k$ coins, corresponding to the possible inputs $\in \{ 0, 1 \}^k$. 
        \item {\bf Position:} The position of a coin is (a lower bound on) the amount of corruption the adversary must've caused so far if Alice's input had indeed been that coin, as a fraction of complete messages.
        \item {\bf Notation:} After round $t$, we denote by $x_i^{(t)}$ the coin in the $i$'th smallest position, where we break ties according to numerical order. We denote by $\pos(y; t)$ the position of coin $y$ after round $t$.
    \end{itemize}
}

With the view that a coin's position is the total amount of corruption so far if Alice's input had actually been that coin, our goal is to show that at the end of the protocol (described below), at most one coin can have position $< T/3$, roughly. 

We now describe the protocol that Alice and Bob engage in. 

\protocol{Constant Round ECC with Feedbck Obtaining Optimal Error Resilience}{1/3-k}{
    Let $T = ?$. 
    
    \begin{itemize} 
    
    \item {\bf Bob's feedback:}
        Each round $t$, Bob's feedback consists of the tuple of $2L_\epsilon$ coins $(x_1^{(t)}, x_2^{(t)}, \dots, x_{2L_\epsilon}^{(t)})$.
        
        For round $0$, it is understood that Bob's ``feedback'' for round $0$ is simply the first $2L_\epsilon$ values of $x \in \{ 0, 1 \}^k$.

    \item {\bf Alice's message:}
        In each round $t$, Alice will send $\ECC_t(x)$, where $\ECC_t$ is a code with certain distance properties depending on Bob's feedback in the previous round. Specifically, $\Delta(\ECC_t(x_{2j-1}^{(t-1)}), \ECC_t(x_{2j}^{(t-1)})) = n_0$ for all $j \in [L_\epsilon]$. And for every $y, z \in \{ 0, 1 \}^k$ with $y \not= z$, it should hold that $\Delta(\ECC_t(y), \ECC_t(z)) \ge (\frac12 - \epsilon) \cdot n_0$. 
    
    \item {\bf Bob's update to the state of the coin game:}
        Upon receiving (possibly corrupted) message $m \in \{ 0, 1 \}^{n_0}$ from Alice in round $t$, Bob will update the state of his coin game by doing the following:
        \begin{enumerate}
            \item 
                He list decodes $m$ to $\ell_t \le L_\epsilon$ values $Y_t = \{ y_{t,1}, \dots, y_{t,\ell_t} \}$ so that $\Delta(\ECC_t(y), m) < (\frac12 - 2\epsilon) \cdot n_0$ for all $y \in Y_t$. 
            \item 
                For each $y \in Y_t$, he increases the position of the corresponding coin by $\frac{\Delta(\ECC_t(y), m))}{n_0}$, so that 
                \[
                    \pos(y; t) = \pos(y; t-1) + \frac{\Delta(\ECC_t(y), m))}{n_0}.
                \]
            \item 
                For each $y \not\in Y_t$, he increases the position of the corresponding coin by $\frac12 - 2\epsilon$, so that 
                \[
                    \pos(y; t) = \pos(y; t-1) + \left( \frac12 - 2\epsilon \right).
                \]
        \end{enumerate}
    
    \end{itemize}
    
    At the end of the protocol, Bob outputs the coin $x_1^{(T)}$. 
}

For ease of reference, we define Bob's update pattern to be the list of updates Bob makes to each coin's position, in order of the current positions of the coins. This will be helpful in the analysis.

\begin{definition}[Update Pattern $(e_1, \dots, e_{2^k})$]
    In round $t$, Bob's \emph{update pattern} in response to message $m$ is defined to be the tuple $(e_1, \dots, e_{2^k})$, where 
    \[
        e_i = \begin{cases}
            \frac{\Delta(\ECC_t(x_i^{(t-1)}), m)}{n_0} & x_i^{(t-1)} \in Y_t \\
            \frac12 - 2\epsilon & \text{otherwise}.
        \end{cases}
    \]
\end{definition}

\begin{remark}
    As we have described it, Bob tracks the positions of all $2^k$ coins. We note that it actually suffices for Bob to track the positions of only $\le T \cdot L_\epsilon$ coins total, since in each of $T$ rounds at most $L_\epsilon$ coins are not increasing their positions by $\frac12 - \epsilon$. In particular, whenever Bob list decodes to a list of coins $Y$, he should begin tracking the coins in $Y$ in addition to the coins he's already tracking. The rest of the coins that he's not tracking will always be understood to be at position $(\frac12 - \epsilon) \cdot t$.
\end{remark}




==> old/brainstorming.tex <==
\subsection{Brainstorming}

General idea for an outline?
\begin{itemize}
    \item Standard ECC solution for error resilience -- capped at 1/4
    \item A way to exploit feedback: coin game
    \item The problem: must specify the order of the coins. Even specifying the first coin is very costly -- $O(k)$ feedback
    \item instead, specify a partition using the indices thing
    \item explain our 1/3 solution; problem: $x_{large}$ will still grow a bit too slowly (highlight how it's different from the odd/even solution of spencer-winkler)
    \item but actually if we remember the normal ECC solution, it exactly succeeds where this fails
    \item Combine the two, and we're basically done
    \item need to send a distance $1$ thing at some point.
\end{itemize}

\noindent
Rachel: Alternative technical overview outline

\begin{itemize}
    \item All existing protocols have $O(k)$ rounds of interaction right now. 
    \item Explain the Spencer-Winkler protocol. Say why is has too many rounds (things can only move by $0$ or $1$ each time, so there's no intermediate separation, so you need $O(k)$ rounds to separate $2^k$ items).
    \item First idea: Alice can send a codeword each time (instead of $0$ or $1$), this way most things will move by some amount, only a few things can move by little. \mnote{distinguish this from the plain ecc solution, maybe by immediately making the proposed solution an ECC where you separate coin 1 and 2 further, rather than mentioning it in the next point.}
    \item Issue is in order to implement this, you need large separation between the first two coins, so you need to specify the first two coins. But this takes $O(k)$ feedback communication.
    \item Instead, with $\log k$ bits of feedback, what you \emph{can} communicate is a partition dividing the first $O(1)$ coins. Explain the coin protocol, say that it gets $x_1 + x_2 + x_3 \ge 1$, which will be enough, since you can send distance $1$ thing at the end (summarize analysis here, postpone discussion of how to prove until later). \mnote{when motivating this new coin game, bring up why the partition solution with x1 and x2 being distance 1 doesnt work, because many coins will move by 0 to say why we can't just use spencer-winkler's idea. this is a bit similar to the xlarge discussion later, so maybe tie it in.}
    \item Issue with this is that the coin game proceeds correctly for the first $O(1)$ coins, but $x_{large}$ grows too slowly and interferes, causing the net growth to be too small.
    \item Instead: only play coin game when $x_{large}$ is far enough away that it doesn't interfere. But how to get $x_{large}$ far away? 
    \item Notice that sending a plain $\ECC$ has the property that $x_{large}$ is moving rapidly. So let's use this so separate! (Note however that sending $\ECC$ by itself is no good, since the close things aren't separating enough. But this will be good enough for us, since we will play $\ECC$ minimally only until $x_3$ and $x_{large}$ are separated.)
    \item Finally, go back and say how pairs analysis works. Main points to hit:
    \begin{itemize}
        \item In Spencer-Winkler analysis, the analysis roughly proceeds by first showing that one attack is always better than the other, then analyzing what happens in that one attack.
        \item Issue for us is that since we have a spectrum of attacks, we can't show in the same way that one attack is better than all the rest and then only analyze that.
        \item Instead, we create the derivative coin game which acts on pairs. The important points: on average pairs are increasing by $\frac23$. For those that aren't increasing by $\frac23$, there's a smaller one that's increasing by more than $\frac23$. 
    \end{itemize}
\end{itemize}

==> old/error-constant-round.tex <==
\section{Constant Round ECCs with Feedback with Optimal Error Resilience}


\protocol{ECC with Feedback Obtaining Optimal Error Resilience in Constant Rounds}{error-constant-rounds}{
    Fix $n\in \bbN$ and $\epsilon>0$ and $N=2^n$ and let Alice's message be $x\in \{0,1\}^n$. The protocol consists of $T = O_\epsilon(1)$ rounds, each of length $M(n)$. In each round, Alice sends a message, followed by which Bob repeats the corrupted message he actually received as feedback to her.
    
    Bob stores a counter for each possible $x\in \{0,1\}^n$ after each round $t$ denoted $\pos(x;t)$. This counter counts the number of bits the adversary would have had to corrupt so far for him to have received the messages he received, if Alice had input $x$\footnote{Note that Bob can correctly compute this quantity because Alice's message in every round is a deterministic function of her input and what Bob received in previous rounds.} divided by $M$ in order to normalize. At the end of the protocol, he outputs the 
    
    To determine 
}

\begin{theorem} \label{thm:error-constant-rounds}
    Protocol~\ref{prot:error-constant-rounds} has $O_\epsilon(1)$ rounds and obtains error resilience $\frac13 - \epsilon$.
\end{theorem}

For $i,j,k \in [N]$, define $\phi_{ijk}(t) = \pos(i; t) + \pos(j; t) + \pos(k; t)$, and let $\phi(t) = \phi_{123}(t) = \min_{ijk} \phi_{ijk}(t)$. Our first goal will be to show that $\phi(T) \approx T$. We start by stating some properties of Bob's update pattern.

\begin{lemma} \label{lemma:e-properties}
    Suppose that Bob updates with weights $e_1, \dots, e_N$. Then:
    \begin{enumerate}
    \item All except for $O_\epsilon(1)$ values of $e_i$ must be at least $\frac12 - 2\epsilon$. 
    \item $e_{2i-1} + e_{2i} = 1$ for all $i \in [N/2]$.
    \item If $e_i \ge \frac12 - 2\epsilon$, then for any distinct $j, k \neq i$ it holds that $e_i + e_j + e_k \ge 1 - 3\epsilon$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    \begin{enumerate}
    \item This claim follows by list decoding \rnote{need to cite this somewhere, also find an actual bound}
    \item $e_{2i-1} + e_{2i} = 1$ follows from the distance properties of the $\ECC$.
    \item Note that all pairs of codewords are distance $\ge \frac12 - \epsilon$ apart. Thus, in particular, $e_j + e_k \ge \frac12 - \epsilon$. Then, $e_i \ge \frac12 - 2\epsilon \implies e_i + e_j + e_k \ge 1 - 3\epsilon$. In particular, there are at most $O_\epsilon(1)$ triples $(i,j,k)$ for which $e_i + e_j + e_k < 1 - 3\epsilon$.
    \end{enumerate}
\end{proof}

\begin{lemma} \label{lemma:triple-bijection}
    For each triple $i < j < k$ such that $e_i + e_j + e_k < 1 - 3\epsilon$, there is another triple $(i', j', k')$ satisfying \rnote{should mention that we consider two triples equivalent if they have the same elements, so order doesn't matter}
    \begin{enumerate}
        \item $(e_i + e_j + e_k) + (e_{i'} + e_{j'} + e_{k'}) \ge 2 - 2\epsilon$.
        \item $i' \le i$, $j' \le j$, and $k' \le k$. In particular, $\phi_{i'j'k'}(t-1) \le \phi_{ijk}(t-1)$.
        \item No two triples $(i,j,k)$ and $(\hat{i}, \hat{j}, \hat{k})$ have the same associated triple $(i', j', k')$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    Consider a triple $i < j < k$ for which $e_i + e_j + e_k < 1 - 3\epsilon$. We define the triple $(i', j', k')$ as follows: 
    \begin{itemize}
        \item $i' = i$. 
        \item Write $j = 2\lfloor \frac{j-1}{2} \rfloor + b$, where $b \in \{ 1, 2 \}$. Then let $j'$ be $\arg\max_{\hat{j} \in \{ j-b, j-b-1 \}} e_{\hat{j}}$. Similarly define $k'$.
    \end{itemize}
    
    First, note that $e_{j'}, e_{k'} \ge \frac12$, since each is the larger of a pair of distances that sum to $1$. Therefore $(e_i + e_j + e_k) + (e_{i'} + e_{j'} + e_{k'}) \ge (e_i + e_j) + (e_i + e_k) + \frac12 + \frac12 \ge 2 - 2\epsilon$. 
    
    Next, note that it's clear that $i' \le i$, $j' \le j$, and $k' \le k$. To show that the associated triple $(i', j', k')$ is unique for each $(i, j, k)$, note that we can perform the reverse mapping, taking a triple $(i', j', k')$ for which $e_{j'}, e_{k'} \ge \frac12$ to a triple $(i, j, k)$ by setting:
    \begin{itemize}
        \item $i = i'$.
        \item Write $j' = 2 \lceil \frac{j'}{2} \rceil - b$, where $b \in \{ 0, 1 \}$. Then let $j = \arg \min_{\hat{j} \in \{ j' + b + 1, j' + b + 2 \}} e_{\hat{j}}$. \rnote{i feel like you need to prove some correctness property also but ima not do that now}
    \end{itemize}
\end{proof}

We now prove the following important property of Protocol~\ref{prot:error-constant-rounds}.

\begin{lemma} \label{lemma:triples}
    For large enough $T = O_\epsilon(1)$, it holds that $\phi(T) \ge (1-4\epsilon)\cdot T$. 
\end{lemma}

\begin{proof}
    Recall that $\phi(T) = \phi_{123}(T) = \pos(1;T) + \pos(2;T) + \pos(3;T)$. 
    
    Consider the following problem: there are $\cN = \binom{N}{3}$ coins corresponding to the triples $i < j < k$ on a board, all beginning at $0$ when $t = 0$. At time $t$, the coin corresponding to $(i, j, k)$ is at position $\phi_{ijk}(t)$. Each round $t$, based on the message that Bob receives, the coin corresponding to $(i, j, k)$ at position $\phi_{ijk}(t-1)$ moves right by $e_i(t) + e_j(t) + e_k(t)$. The adversary's goal is to cause the leftmost \rnote{define leftmost?} coin to be at a position $< T - ?$ at time $T$.
    
    \rnote{insert lemma that you can always make the $e_i$ smaller}
    
    Thus, by Lemma~\ref{lemma:e-properties} and Lemma~\ref{lemma:triple-bijection}, it suffices to consider sequences of update weights $w_1, \dots, w_\cN$ for which for each of $O_\epsilon(1)$ many $i$ for which $w_i < 1 - 3\epsilon$, there exists $i' < i$ (unique to $i$) such that $w_i + w_{i'} = 2 - 6\epsilon < 2-2\epsilon$, and for all other $i$ it holds that $w_i = 1-3\epsilon$. \rnote{should say that we are reindexing to look at $[\cN]$}
    
    Consider the following potential function 
    \[
        F(t) = \sum_{i \in [\cN]}(1 + \epsilon)^{4|\phi_i(t)-(1-3\epsilon)t|} - (\cN - T \cdot O_\epsilon(1)).
    \]
    Note that at time $t = 0$, $\phi_i(0) = 0$ for all $i \in \cN$, so $F(t) = T \cdot O_\epsilon(1)$. Furthermore, at time $t$, note that at most $T \cdot O_\epsilon(1)$ of the coins are not at $(1-3\epsilon)t$, since each round $O_\epsilon(1)$ of the $i$ have $w_i \not= 1 - 3\epsilon$.
    
    Consider an update weight $w_i$ and its associated update weight $w_{i'}$ such that $i' < i$ and $w_i + w_{i'} = 2 - 6\epsilon$. Write $w_i = 1 - 3\epsilon - \delta$, and $w_{i'} = 1 - 3\epsilon + \delta$, and denote $d_i(t) = \phi_i(t) - (1-3\epsilon) \cdot t$. At time $t-1$ these two coins contribute 
    \[
        (1+\epsilon)^{4|d_i(t-1)|} + (1+\epsilon)^{4|d_{i'}(t-1)|} 
    \]
    to $F(t-1)$. If either $|d_i(t-1)| \ge \delta$ or $|d_{i'}(t-1)| \ge \delta$, then note that after round $t$ the larger of $|d_i(t-1)|, |d_{i'}(t-1)|$ will decrease by a multiplicative factor of $(1+\epsilon)^{4\delta}$, and the smaller of $|d_i(t-1)|, |d_{i'}(t-1)|$ will increase by at most a multiplicative factor of $(1+\epsilon)^{4\delta}$. In particular, 
    \[
        (1+\epsilon)^{4|d_i(t)|} + (1+\epsilon)^{4|d_{i'}(t)|} \le \frac{(1+\epsilon)^{4\delta} + (1+\epsilon)^{-4\delta}}{2} \cdot \left( (1+\epsilon)^{4|d_i(t-1)|} + (1+\epsilon)^{4|d_i(t-1)|} \right).
    \]
    We also have that $\delta \le \frac14$ \rnote{need to prove this rigorously also} because of 3-way list decoding, so the above simplifies to 
    \begin{align*}
        (1+\epsilon)^{4|d_i(t)|} + (1+\epsilon)^{4|d_{i'}(t)|} 
        &\le \frac{(1+\epsilon) + (1+\epsilon)^{-1}}{2} \cdot \left( (1+\epsilon)^{4|d_i(t-1)|} + (1+\epsilon)^{4|d_i(t-1)|} \right) \\
        &\le e^{\epsilon^2/2} \cdot \left( (1+\epsilon)^{4|d_i(t-1)|} + (1+\epsilon)^{4|d_i(t-1)|} \right).
    \end{align*}
    \rnote{need to make above more rigorous}
    If both $|d_i(t-1)|, |d_{i'}(t-1)| < \delta$, then after round $t$ the two coins will contribute an additive additional
    \begin{align*}
        \left( (1+\epsilon)^{4(\delta - |d_i(t-1)|)} + (1+\epsilon)^{4(\delta - |d_{i'}(t-1)|)} \right) - \left( (1+\epsilon)^{4|d_i(t-1)|} + (1+\epsilon)^{4|d_{i'}(t-1)|} \right)
        &\le 2 \cdot (1+\epsilon)^{4\delta} - 2 \\
        &\le 2\epsilon.
    \end{align*}
    
    Combining the two above observations, we have that 
    \[
        F(t) \le e^{\epsilon^2/2} F(t-1) + O_\epsilon(1).
    \]
    Solving, we get that $F(T) \le C_\epsilon \cdot e^{T\epsilon^2/2}$. \rnote{not sure if exactly correct} 
    
    Finally, note that at time $T$ a chip at position $\phi_i$ will contribute $(1+\epsilon)^{4|\phi_i - (1-3\epsilon)\cdot T|}$ to $F(T)$. So in particular, let $\phi$ be the smallest position of the $\cN$ chips. Then 
    \begin{align*}
        (1+\epsilon)^{4|\phi - (1-3\epsilon)\cdot T|} &\le C_\epsilon \cdot e^{T\epsilon^2/2} \\
        \implies 4|\phi - (1-3\epsilon)\cdot T| \le \frac{1}{\ln (1+\epsilon)} \cdot \left( \ln C_\epsilon + T\epsilon^2/2 \right) \\
        \implies \phi \ge (1 - 3\epsilon) \cdot T - \frac{1}{4 \cdot \epsilon/2} \cdot \left( \ln C_\epsilon + T \epsilon^2/2 \right) 
        = (1 - 3\epsilon) \cdot T - \frac{\ln C_\epsilon}{2\epsilon} - \frac{\epsilon T}{4}.
    \end{align*}
    Now if we choose $T = O_\epsilon(1)$ large enough, the bound follows.
    
\end{proof}

We can now prove Theorem~\ref{thm:error-constant-rounds}.

\begin{proof}[Proof of Theorem~\ref{thm:error-constant-rounds}]
    Suppose for the sake of contradiction that there is some sequence of messages that Bob could receive such that $\pos(1; T), \pos(2; T) < \frac{1-4\epsilon}{3} \cdot T$. 
    
    Consider the potential function 
    \[
        \Psi(t) = \pos(1; t) + \pos(2; t) + \min(\pos(3; t), \frac{1-4\epsilon}{3} \cdot T).
    \]
    According to Lemma~\ref{lemma:triples}, as long as $\pos(3; t) < \frac{1-4\epsilon}{3} \cdot T$, $\Psi(t)$ increases by $\ge 1 - 4\epsilon$ each round. After $\pos(3; t) \ge \frac{1-4\epsilon}{3} \cdot T$, by assumption we always have that $\pos(1;t), \pos(2; t) < \frac{1-4\epsilon}{3} \cdot T$ so there can be no crossover with other coins, thus since the first two coins' distances must always add up to $1$, $\Psi(t)$ increases by $1$ each time. Therefore, $\Psi(T) \ge (1-4\epsilon) \cdot T$. But this is a contradiction with $\pos(1; t), \pos(2; t) < \frac{1-4\epsilon}{3} \cdot T$. 
\end{proof}


==> old/error-log-bits.tex <==
\begin{theorem}
Any protocol 
\end{theorem}

\protocol{ECC with Feedback Obtaining $\frac27$ Error Resilience in Constant Rounds and $\log$ bits}{error-constant-rounds}{
    Fix $n\in \bbN$ and $\epsilon>0$ and let Alice's message be $x\in \{0,1\}^n$.
}

==> old/error-old.tex <==
\subsection{Feedback ECC for Errors} \label{sec:overview-error}

\vnote{Mention there are two approaches: rewind with error, and partition based. Quickly dismiss former as not suitable, but do mention HKV even if it's not that interesting for our goals.}

\vnote{For the overview, it might be easier to follow to first give a description of SW protocol and then with that context available, describe the changes, and highlight the most important/subtle aspects, such as the use of list-decodable codes and need for distance within $P_1$ itself. The former might not be not novel any more given your previous works, but perhaps the latter and the overall combination will stand out as novel techniques in this work.}

We begin with the coin game reformulation of~\cite{Berlekamp64,SpencerW92}. In the coin game setup, there are $2^k$ coins corresponding to the $2^k$ possible values of Alice's input on a board. At the beginning of the game, all coins are at position $0$. Throughout the game, Alice sends Bob a message, after which Bob updates the positions of all coins on the board. At any point in the game, the position of a coin on the board should be the amount of corruption the adversary must've caused had Alice's input actually been that coin. We say that a coin falls off the board if its position exceeds $T/3$, where $T$ is the total number of rounds of communication. Note that if a coin is still on the board after the $T$ rounds, then it could have plausibly been Alice's input given that the adversary corrupted $< T/3$ of Alice's communication. The goal is to design Alice's messages in response to Bob's feedback in such a way that only one coin can remain on the board after $T$ rounds.

In the feedback ECCs of~\cite{Berlekamp64,SpencerW92} \rnote{more references?}, every round Bob sends Alice as feedback a partition of the $2^k$ coins into two\footnote{In the works of~\cite{Berlekamp64} \rnote{more references}, the coins are actually partitioned into 3 sets.} sets, which Alice responds to by telling Bob which partition her input belongs to. In particular, Alice's message is always a single bit, $0$ or $1$, denoting the correct partition. Thus, the only thing the adversary can do is either change which partition Bob receives, or allow him to receive the correct partition.

Even without corruption, in order to single out a single element of $\{ 0, 1 \}^k$, there needs to be $\log 2^k = k$ rounds of communication. It is instructive to see what is happening in the coin game reformulation. In the coin game view, every round Bob increases the positions of the $2^k/2$ coins in the partition opposite to the one he received by $1$, while keeping the other $2^k/2$ coins at the same position. Thus, after round $i$, $2^k/2^i$ of the coins will still be lagging at position $0$. This means that there must be at least $k$ rounds. \mnote{I think the ordering of sentences in the last couple paragraphs is a bit weird. i think talk about how eve basically gets to choose a set of coins to move at each step before introducing complexity and then discuss the reason for $k$ rounds}

\paragraph{Idea 1: Sending an ECC.}

Our first observation is that if Alice were instead sending $\ECC(x)$, where $\ECC$ is an error correcting code and relative distance $\frac12$, then after a single round, \emph{only one coin} can still be at position $0$. Actually, this is not quite enough: in order for a coin to fall off the board by time $T$, its position must increment by $\frac13$\footnote{Here, in the technical overview, we will view positions in the coin game as a fraction of total Alice messages corrupted, so corrupting an entire $\ECC(x)$ will increment a coin's position by $1$. This will be different than our description in Section~\ref{sec:error}, in which the coin game will count an explicit number of bit corruptions, so corrupting an entire $\ECC(x)$ will increment a coin's position by $M$.} every round, so we really care that there aren't too many coins that increment by less than $\frac13$. Indeed, this is given to us by the list-decoding guarantees of $\ECC$: at most $O(1)$ coins will increment by less than $\frac12$! Thus, since only $O(1)$ coins can lag below $\frac13$ (in fact, $\frac12$) each round, it seems plausible that it would only take constant rounds to separate out a single coin.

However, note the following issue with simply having Alice send $\ECC(x)$ each round. Since the best relative distance for a binary code is $\frac12$, meaning that there exist two codewords, say $\ECC(x)$ and $\ECC(y)$, for which only $\frac12$ of the bits differ, an adversary could simply corrupt Alice's communication every round so that it is relative distance $\frac14$ from both $\ECC(x)$ and $\ECC(y)$. Then, by the end of the protocol, both coins $x$ and $y$ are at position $\frac{T}4$, so that Bob cannot distinguish between the two. 

To get around this, it is important to use an $\ECC$ such that the distance between $\ECC(x_1)$ and $\ECC(x_2)$ is large, where $x_1$ and $x_2$ are the coins with the smallest and second smallest positions on the board at a given timestep, respectively. To allow this, Bob can send $x_1$ and $x_2$ in every round, which allows Alice to use the appropriate $\ECC$ for her next message. 

However, note that sending over $x_1$ and $x_2$ requires $2k$ bits of feedback from Bob, which is too much for us (recall that we want $O(\log k)$ total bits of feedback). Thus, we will need to reduce the amount of information Bob is sending. \mnote{random english comment: the phrase "note that" is used a lot.} \mnote{I find the presentation of the "ECC Idea" a little weird because it's literally just ignoring feedback and sending an ECC, and so is not really a strategy; maybe makes more sense to say "let's look at sending an ECC in view of the coin game, and see what happens. we get most things moving by $\frac12$ but a few things that move very slowly, potentially all by $\frac14$.}

\paragraph{Idea 2: Bob sends a short description of a partition of $\{ 0, 1 \}^k$.}

While Bob \emph{cannot} send the elements $x_1$ and $x_2$, what he \emph{can} send is a short description of a partition of $\{ 0, 1 \}^k$ separating $x_1$ and $x_2$ into different sets of the partition. The idea is that while he can't explicitly specify $x_1$ and $x_2$, the partition is enough information so that Alice's next $\ECC$ can separate out $x_1$ from $x_2$. To do this, Bob chooses an index $i \in [k]$ for which $x_1[i] \not= x_2[i]$, and sends to Alice $(i, x_1[i], x_2[i])$. Note that this is $\log k + 2$ bits total. 

Using feedback $(i, b_1, b_2)$, where $b_1 \not= b_2 \in \{ 0, 1 \}$, Alice can determine the partition, where the first set $P_1$ consists of all $y \in \{ 0, 1 \}^k$ for which $y[i] = b_1$ and the second set $P_2$ consists of all $y \in \{ 0, 1 \}^k$ for which $y[i] = b_2$. Note that $x_1 \in P_1$ and $x_2 \in P_2$. Then Alice can send $\ECC(x)$, where $\ECC$ satisfies that $\Delta(\ECC(y_1), \ECC(y_2))$ is large for all $y_1 \in P_1$ and $y_2 \in P_2$. \mnote{why are $b_1$ and $b_2$ necessary to send?}

\paragraph{Observation:} In~\cite{SpencerW92}'s protocol, it is vital to the analysis that Alice's messages for $x_1$ and $x_2$ are separated by relative distance $1$. For us, if Alice's $\ECC$ satisfies that $\Delta_{rel}(\ECC(x_1), \ECC(x_2)) = 1$, it must hold that there is a fixed codeword $C_1$ such that $\ECC(y) = C_1$ for all $y \in P_1$, and $\ECC(y) = C_2 = \overline{C_1}$ for all $y \in P_2$, where $\overline{C_1}$ denotes the result of flipping every bit of $C_1$. Then, every round, depending on the adversary's corruption, the positions of all the coins in $P_1$ will increment by $\delta$, while the positions of all the coins in $P_2$ will increment by $1-\delta$. 

However, this seems to lead to a similar problem as earlier: in each round the position increments of half the coins each round can lag behind, so that a total of $O(k)$ rounds will be needed to single out a coin. \mnote{As commented later, though this is technically an issue too, the much bigger issue is the protocol is that xlarge moves by $0$. maybe this is the same thing actually im not sure, but xlarge moving by $0$ motivates the protocol better.}

\paragraph{Idea 3: Smallest three coin positions increasing at $\gtrsim 1$ suffices.} 

Instead, we note that in the analysis of~\cite{SpencerW92}, the fact that $\ECC(x_1)$ and $\ECC(x_2)$ have relative distance $1$ becomes important only after all other coins have already dropped off the board. Before that, it is important only that the three smallest positions of coins on the board is increasing at $\gtrsim 1$ each round (note that the particular coins with the three smallest positions may change between rounds). Concretely, Spencer and Winkler are concerned with the potential function $\Phi(t) = \posx(1; t) + \posx(2; t) + \min \{ T/3, \posx(3; t) \}$, where $\posx(i; t)$ denotes the $i$'th smallest position of a coin after round $t$. Suppose that $T_1$ is the smallest round after which $\posx(3; T_1) \ge T/3$. Then before round $T_1$, $\Phi(t)$ grows at $\gtrsim 1$ each round, so that $\Phi(T_1) \gtrsim T_1$. After round $T_1$, since $\ECC(x_1)$ and $\ECC(x_2)$ are relative distance $1$ apart, the position increments of $x_1$ and $x_2$ must sum to $1$, so that $\Phi(t)$ continues increasing at $1$ each round. Then, after round $T$, $\Phi(T) = \posx(1; t) + \posx(2; t) + \min \{ T/3, \posx(3; t) \} \gtrsim T$, implying that $\posx(1; t) + \posx(2; t) \gtrsim 2T/3$, or that only one coin can still have position $\lesssim T/3$. 

For us, as long as we can devise a feedback ECC in which the positions of the three smallest coins are increasing by $\gtrsim 1$ each round, then as soon as all but two coins have fallen off the board, we can switch to having Alice send $\ECC(x)$ such that $\Delta_{rel}(\ECC(x_1), \ECC(x_2)) = 1$ to separate out the last two coins remaining on the board. This can be done with low feedback communication: Bob can simply send an index $i$ ($\log k$ bits) for which $x_1[i] \not= x_2[i]$, and Alice's message will just be $x[i]$. 

Therefore, we reduce now to devising a protocol where $\posx(1; t) + \posx(2; t) + \posx(3; t)$ is increasing by $\gtrsim 1$ each round, but only $O(1)$ rounds are needed. \mnote{I sort of feel like this secion can be shorter, it's restated/concluded like 3 times that we want a protocol where 1+2+3 is increasing at a rate of 1. I think it suffices to say something like: It suffices to have a protocol where 1+2+3 increases by 1. As long as we have such a protocol, then as soon as all but two coins have fallen..." and mention that the idea is from SW.}

\paragraph{A constant round feedback ECC with three smallest coin positions increasing by $\gtrsim 1$.}

Let $x^t(i)$ denote the coin with the $i$'th smallest position after round $t$. Fix coins $x_1, \dots, x_c$ to the coins $x^{T_0}(1), \dots, x^{T_0}(c)$ after some round $T_0$, where $c = O(1)$. Consider the following protocol between Alice and Bob for rounds $t > T_0$, given in Protocol~\ref{prot:protocolB}.

\protocol{Feedback ECC Candidate}{protocolB}{
\begin{itemize}
\item 
    Every round $t > T_0$, Bob will send to Alice a list of $c$ indices $i_1, \dots, i_c$ along with the values of $x_i[i_1, \dots, i_c]$ for each $i \in [c]$. This specifies a partition of $\{ 0, 1 \}^k$ into three sets as follows: 
    \begin{itemize}
    \item 
        $P_1$ consists of all $y \in \{ 0, 1 \}^k$ for which $y[i_1, \dots, i_c] = x_i[i_1, \dots, i_c]$,
    \item 
        $P_2$ consists of all $y \in \{ 0, 1 \}^k$ for which $y[i_1, \dots, i_c] = x_j[i_1, \dots, i_c]$ for some $j = 2, 4, 6, \dots$,
    \item 
        $P_3$ consists of all $y \in \{ 0, 1 \}^k$ for which $y[i_1, \dots, i_c] = x_j[i_1, \dots, i_c]$ for some $j = 3, 5, 7, \dots$.
    \end{itemize}
    All other $y \in \{ 0, 1 \}^k$ can be thrown into an arbitrary partition, say $P_1$.
    
\item 
    Alice responds by sending $\ECC(x)$, where $\ECC$ is a code with the following distance properties:
    \begin{itemize}
        \item $\Delta_{rel}(\ECC(y_1), \ECC(y_2)) \ge \frac13$ for all $y_1 \not= y_2 \in P_1$. 
        \item There is some fixed codeword $C_2$ such that $\ECC(y) = C_2$ for all $y \in P_2$.
        \item There is some fixed codeword $C_3$ such that $\ECC(y) = C_3$ for all $y \in P_3$. 
        \item For any $y_1, y_2$ in different partition sets, $\Delta_{rel}(\ECC(y_1), \ECC(y_2)) \ge \frac23$.
    \end{itemize}
    Such an $\ECC$ is shown to exist in Claim~\ref{claim:ecc3}.
\end{itemize}
}

It turns out (as we will discuss in Section~\ref{sec:overview-minigame}) that the three smallest positions among $x_1, \dots, x_c$ will increase by $\gtrsim 1$ each round! % In fact, something even stronger is true: that the two smallest positions will increase by $\gtrsim \frac23$ each round. 

However, the same is not true once you consider the rest of the $2^k$ coins as well. For instance, consider the adversary who corrupts the communication so that Bob receives $\ECC(x_1)$ every round. Then, while the positions of each of $x_2, \dots, x_c$ increases by $\frac23$ every round, the positions of other elements in $P_1$ are only increasing by $\frac13$. Then, after sufficiently many rounds, the coins $x_2, \dots, x_c$ have passed (have larger positions than) the coins in $P_1$, and the sum of the positions of the first three coins will thereafter only increase by $\frac23 = 0 + \frac13 + \frac13$ each round. This will not suffice. \vnote{The last couple of sentences are hard to follow.}

Instead, we only play Protocol~\ref{prot:protocolB} when the position of $x_{large}$ is sufficiently large that the smallest three positions among $x_1, \dots, x_c$ won't pass it. (Here, $x_{large} = x^{T_0}(c+1)$ is the position of the smallest coin not explicitly separated out by the partition.) 

The question then is how do we ever enter a state in which $x_{large}$ is sufficiently larger than $x_3$? Clearly, playing Protocol~\ref{prot:protocolB} from the beginning will not work. 

\paragraph{Idea 4: Combining the ECC solution and Protocol~\ref{prot:protocolB}.}

Notice that sending a plain $\ECC$ (with relative distance $\frac12$), as we proposed earlier, has the property that $x_{large}$ moves rapidly, at rate $\frac12$ per round. We thus propose the following procedure:
\begin{itemize}
    \item 
        If $x_{large}$ and $x_3$ are close together, Alice sends $\ECC(x)$, where $\ECC$ is a standard error correcting code with relative distance $\frac12$, until the position of $x_{large}$ is sufficiently larger ($\approx \epsilon T$) than the position of $x_3$. 
    \item 
        Once the position of $x_{large}$ is sufficiently larger than that of $x_3$, Alice and Bob engage in Protocol~\ref{prot:protocolB} instead. They do this until $x_{large}$ and $x_3$ become close together \mnote{again}.
\end{itemize}

The point then is that whenever Alice is sending $\ECC(x)$ using the plain $\ECC$, the position of $x_{large}$ is a good approximation for the position of $x_3$. Furthermore, it is not hard to show that the positions of $x_1$, $x_2$, and $x_{large}$ grows at roughly $1$ per round while Alice is sending $\ECC(x)$: the position of $x_{large}$ is growing at $\frac12$ per round due to the list decoding guarantee of $\ECC$, and the codewords associated with $x_1$ and $x_2$ have distance $\frac12$, so that the combined positional increase is $\frac12 + \frac12 = 1$.

Thus, whether Alice is sending $\ECC(x)$ using a standard error correcting code or engaging in Protocol~\ref{prot:protocolB}, the three smallest positions of coins on the board is increasing at rate $1$ per round. \mnote{hm, i don't think theres any explanation of why xlarge grows at 1/3 instead of 0, which is probably the main idea of the protocol. I think one way to help with this is going back to the 0/1/0/1 approach, and it's bad because xlarge grows by 0 if you can't truly alternate the coins after xlarge. this problem is still present in the new appraoch, until you bring in the list decoding making xlarge grow fast. In general, i feel the first 3 ideas are overexplained, but the feedback ECC candidate + idea 4 is underexplained.}

For the formal statement and analysis of our protocol, we refer the reader to Section~\ref{sec:error}.


\input{overview/coin-minigame}






==> old/lower-bound-randomized.tex <==
\section{Lower Bound on the Number of Bits of Feedback}

For error correcting codes without feedback, it is well known the maximum error (resp. erasure) resilience the parties can achieve is $\frac14$ (resp. $\frac12$). Suppose that Alice has input $x \in \{ 0, 1 \}^k$, which she is trying to convey to Bob with feedback from Bob. Here we show that Bob must send at least $\Omega(\log{n})$ bits of feedback in order to surpass this threshold. With only $o(\log{n})$ bits of feedback, the parties cannot achieve higher error resilience than they could without feedback.

\begin{theorem}
    For any $\delta>0$, any randomized feedback ECC family $\{\code\}_{k\geq 0}$ that achieves error resilience $\frac14 +\delta$ requires $\Omega(\log{k})$ bits of feedback. Similarly, any $\code$ that achieves erasure resilience $\frac12 +\delta$ requires $\Omega(\log{k})$ bits of feedback.
\end{theorem}

\begin{proof}
    Throughout the proof, fix $k$ and let $\code$ denote $\code_k$. Let Alice and Bob's private randomness both be drawn from $\{0,1\}^R$ for some $R\in \bbN$. Let $G$ be the complete graph whose vertices are Alice's possible messages. We denote the vertices $v_1\ldots v_K$ where $K=2^k$. On each input $v_1\ldots v_K$, let $\code(v_i,f,r)$ denote the sequence of bits Alice sends throughout the protocol, where $f\in \{0,1\}^{|\code|_f}$ denotes the feedback messages she gets from Bob, and $r \in \{0,1\}^R$ denotes Alice's private randomness. Let $\code_{-1}(v_i,f,r) = 2\code(v_i,f,r)-\mathbb{1}$, in words a relabeling of the alphabet $\{0,1\}$ to $\{-1,1\}$. 
    
    In the graph $G$, we label the edge $v_i-v_j$ with $f\in \{0,1\}^{|\code|_f}$ if if $f$ is the lexicographically first string for which the following holds:
    \[
        \E_{r_i\in \{0,1\}^R}\left[\code_{-1}(v_i,f,r_i)\right]\cdot \E_{r_j\in \{0,1\}^R}\left[\code_{-1}(v_j,f,r_j)\right] < -10\delta
    \]
    
    We show that if there is an unlabeled edge, then Eve has an attack, where Bob guesses incorrectly with probability at least $0.01\delta$. In order to output Alice's message with probability $>1-0.01\delta$, Bob's algorithm must solve a simpler task: given (corrupted) messages from Alice who either has input $i$ and randomness $r_i\in \{0,1\}^R$ or input $j$ and randomness $r_j\in \{0,1\}^R$ where $i<j$, output which case with probability at least $1-0.02\delta$ over $r_i,r_j$ and Bob's randomness $r$. Otherwise, 
    \[
        \Pr_{r_i,r_j,r}[\text{Bob guesses $v_i$ when Alice has $v_j$}] + \Pr_{r_i,r_j,r}[\text{Bob guesses $v_j$ when Alice has $v_i$}] \geq 0.02\delta
    \]
    so one of the two values is at least $0.01\delta$, which implies that Bob guesses incorrectly on that input with probability at least $0.01\delta$.
    
    The proof that Bob's algorithm cannot solve this simpler problem is separate for the case of errors and the case of erasures.
    
    \paragraph{Errors.} Fix Bob's randomness $r$. We show that with probability $0.02\delta$ over $r_i,r_j\in \{0,1\}^R$, Eve can corrupt both versions of Alice (whom we call Alice$_i$ and Alice$_j$ to send the same message (without knowing $r_i$ or $r_j$ in advance. She corrupts Alice$_j$'s messages to match Alice$_i$ until this required $\frac14+\delta$ corruption from Alice$_j$. Then, she corrupts Alice$_i$'s messages 
    
    \paragraph{Erasures.} Again, fix Bob's randomness $r$. We show that with probability $0.02\delta$ over $r_i,r_j\in \{0,1\}^R$, Eve can corrupt both versions of Alice to send the same message.
    
    Thus, we have shown that every edge of the graph $G$ has a label. We now show that there is no $K_{\lceil 10/\delta\rceil}$ with the same label on all edges. Assume for the sake of contradiction that $v_{i_1}\ldots v_{i_{\lceil 10/\delta\rceil}}$ is a complete subgraph. Then 
    \begin{align*}
        &~ \left|\sum_{a=1}^{\lceil 10/\delta\rceil} \E_{r} [C_{-1}(v_{i_a}, f, r)]\right|^2 \geq 0 \\
        \implies &~ \sum_{a=1}^{\lceil 10/\delta\rceil} \left|\E_{r} [C_{-1}(v_{i_a}, f, r)]\right|^2 \geq -\sum_{a\neq b} \E_{r_a, r_b} [C_{-1}(v_{i_a}, f, r_a) \cdot C_{-1}(v_{i_b}, f, r_b)] \\
        &~ \geq \lceil 10/\delta\rceil \cdot (\lceil 10/\delta\rceil-1)\cdot 10\delta \geq \frac{500}{\delta}
    \end{align*}
    
    Notice that for all $a$, it holds that $|\E_{r} [C_{-1}(v_{i_a}, f, r)]|^2\leq 1$, so the left hand expression is at most $\lceil 10/\delta\rceil$, which is a contradiction.
    
    Therefore, we can view the labeling of $G$ as a coloring of the edges avoiding $K_{\lceil 10/\delta\rceil}$. By a well-known bound on multicolor Ramsey numbers, the number of labels necessary for a graph on $K$ vertices is $\Omega\left(\frac{\log{K}}{\log\log{K}}\right)$. Therefore, the number of possibilities for $f$ must be $\Omega\left(\frac{\log{K}}{\log\log{K}}\right)$, so the number of feedback bits transmitted by Bob is at least $\log{\Omega\left(\frac{\log{K}}{\log\log{K}}\right)}=\Omega{\log{k}}$.
\end{proof}

==> overview/other-protocols.tex <==
We begin by showcasing the Spencer-Winkler protocol \cite{SpencerW92} that achieves an error resilience of $\frac13$ using $O(k)$ rounds and bits of feedback. 

\subsection{The Spencer-Winkler Coin Game} \label{sec:other-prot}

\paragraph{The Coin Game:} The second approach is the coin game of \cite{Berlekamp64,SpencerW92}. In the coin game setup, there are $2^k$ coins corresponding to the $2^k$ possible values of Alice's input on a board. At the beginning of the game, all coins are at position $0$. Throughout the game, Alice sends Bob a message, after which Bob updates the positions of all coins on the board with the amount of corruption Eve would have needed to use in that message if Alice actually had that coin as her input. If the protocol has $T$ bits, a coin falls off the board if its position exceeds $T$. The goal is to design Alice's messages in response to Bob's feedback in such a way that only one coin can remain on the board after $T$ rounds, regardless of what Eve corrupts Alice's messages to.

Specifically, the protocol of \cite{SpencerW92} is as follows. At every step, Bob tells Alice an ordering of his coins from smallest to largest position value (breaking ties arbitrarily). Alice sends him $0$ if her input is an odd numbered coin according to this ranking, and $1$ if her input has an even ranking. To analyze this protocol, let $\posx(i)$ denote the position of the $i$'th coin in this ranking. It turns out that regardless of whether Eve chooses to move the even or odd coins each up by $1$, the quantity $\posx(1)+\posx(2)+\posx(3)$ increases by $\gtrsim 1$ at each step, which Spencer and Winkler showed using a concentration inequality argument, taking $O(k)$ rounds to converge. This shows directly that at least one coin falls off the board (exceeds $|T|/3$) by the end of the protocol. As soon as the third coin falls off the board, the even/odd strategy additionally causes $\posx(1)+\posx(2)$ to increase by $\gtrsim 1$ at each step as long as both stay on the board, and ultimately this ensures that the second coin falls off the board as well.


